Previous Knowledge Utilization In Online Anytime Belief Space Planning

Online planning under uncertainty remains a critical challenge in robotics and autonomous systems. While tree search techniques are commonly employed to construct partial future trajectories within computational constraints, most existing methods discard information from previous planning sessions considering continuous spaces. This study presents a novel, computationally efficient approach that leverages historical planning data in current decision-making processes. We provide theoretical foundations for our information reuse strategy and introduce an algorithm based on Monte Carlo Tree Search (MCTS) that implements this approach. Experimental results demonstrate that our method significantly reduces computation time while maintaining high performance levels. Our findings suggest that integrating historical planning information can substantially improve the efficiency of online decision-making in uncertain environments, paving the way for more responsive and adaptive autonomous systems.

==> 05-mcts_planning.tex <==
\section{MCTS Planning With Calculation Re-Use}
\subsection{MCTS notations}
The PFT algorithm \cite{Sunberg18icaps} uses Monte-Carlo simulation and constructs incrementally a policy tree. For each belief node $b_k$ and action $a_k$ it defines visitation count $N(b_k,a_k)$, $N(b_k)=\sum_{a}N(b_k,a_k)$ and value $Q(b_k,a_k)$ which is the average accumulated reward when starting from the node $b_k$ and executing action $a_k$. The generation of a new posterior belief is made using particle filter method  $\SB{k+1},\SPB{k+1},r \leftarrow G_{PF(m)}(b_k,a_k)$ and in the process a new propagated belief $\SPB{k+1}$ is created. We define $Q(\SPB{k+1})$ as the average accumulated reward starting from the node $\SPB{k+1}$ and by definition $Q(b_{k+1},a_k)=\sum_{\SPB{k+1} \in C(b_k,a_k)}Q(\SPB{k+1})$ where $ C(b_k,a_k)$ marks all of the propagated beliefs we have so far when applying action $a_k$ in belief $b_k$. We define  $\tau_{i}(\SB{k},a_k)$ as a trajectory 
\begin{multline}
	\tau_{i}(\SB{k},a_k) \triangleq  (\SB{k},a_k)\rightarrow (b^{-i}_{k+1},b^{i}_{k+1},a^i_{k+1}) \rightarrow ... \hfill \\ \rightarrow (b^{-i}_{k+d},b^{i}_{k+d},a^i_{k+d}) \hfill
\end{multline}															
where $k+d$ marks the horizon.

\begin{theorem} \label{th:trajectory_likelihood_ratio}
	\textit{Given two trajectories  $\tau_{1}(\SB{k},a_k)$
		and $\tau_{2}(\SB{k}',a_k')$ with planning horizon  $d>0$ that differs only in the first belief $b$ and action $a$, \\ $\tau_{1}(\SB{k},a_k) \triangleq (\SB{k},a_k)\rightarrow (b^{-}_{k+1},b_{k+1},a_{k+1}) \rightarrow ... \rightarrow (b^-_{k+d},b_{k+d},a_{k+d})$. \\ $\tau_{2}(\SB{k},a_k) \triangleq (\SB{k}',a'_k)\rightarrow (b^{-}_{k+1},b_{k+1},a_{k+1}) \rightarrow ... \rightarrow (b^-_{k+d},b_{k+d},a_{k+d})$. The likelihood ratio of the trajectories is equal to the likelihood ratio of the first propagated beliefs
		$\frac{\prob(\tau_{1}(\SB{k},a_k))}{\prob(\tau_{2}(\SB{k}',a'))}=\frac{\prob(a_k|b_k,\pi_k)\prob(\SPB{k+1}|b_k,a_k)}{\prob(a'_k|b'_k,\pi'_k)\prob(\SPB{k+1}|b'_k,a'_k)}$}.
	\small
\end{theorem}

\subsection{Multiple-Importance Sampling in MCTS}
We start with writing explicitly the term $Q(\SB{k},a_k)$

\begin{multline} \label{eq:q_func_mcts}
	Q(\SB{k},a_k) = \frac{1}{N(\SB{k},a_k)} \sum_{i=1}^{N(\SB{k},a)}q(\tau_{i}(\SB{k},a)) \hfill 
\end{multline}
where $\tau_{i}(\SB{k},a_k)$ is a trajectory of the form $(\SB{k},a_k)\rightarrow (\SPB{k+1},\SB{k+1},a_{k+1}) \rightarrow ... \rightarrow (\SPB{k+d},\SB{k+d},a_{k+d})$, $q(\tau_{i}(\SB{k},a_k)) = \sum_{j=0}^{d-1}r(\SB{k+j},a_{k+j}, \SB{k+j+1})$.
 Using eq \ref{eq:multiple_importance_sampling} and Theorem \ref{th:trajectory_likelihood_ratio} we define Multiple-Importance Sampling estimator $Q_{MIS}(\SB{k},a_k)$ of $Q(\SB{k},a_k)$ from Eq \ref{eq:q_func_mcts} \VI{[reduce the derivations below,  move to appendix (for the paper, can leave in the thesis)]}

\begin{multline} \label{eq:q_mcts_mis}
	Q_{MIS}(\SB{k},a_k) = \sum^{M}_{m=1}\frac{1}{ N(\SPB{k+1,m})} \cdot \hfill \\
	\sum^{ N(\SPB{k+1,m})}_{i=1}w_{m}(\tau_{i,m})  \frac{p(\tau_{i,m})}{q_{m}(\tau_{i,m})}
	q(\tau_{i,m}(\SB{k},a_k)) =  \hfill \\
	\sum^{M}_{m=1}\frac{1}{ N(\SPB{k+1,m})} \cdot \hfill \\
	\sum^{ N(\SPB{k+1,m})}_{i=1}w_{m}(\tau_{i,m})  \frac{\prob(a_k|b_k,\pi_k)\prob(\SPB{k+1}|b_k,a_k)}{\prob(a'_k|b'_k,\pi'_k)\prob(\SPB{k+1}|b'_k,a'_k)}
	q(\tau_{i,m}(\SB{k},a_k))\hfill
\end{multline}
We choose the balance heuristic \cite{Veach95siggraph} for the weights
$w_m(\tau_{i,m})=\frac{N(\SPB{k+1,m}) p(\tau_{i,m}(b_k,a_k))}{\sum^{M}_{j=1}N(\SPB{k+1,j}) q_j(\tau_{i,m}(b_k,a_k))} = \frac{N(\SPB{k+1,m}) \prob(a_{k_m}|b_{k_m},\pi_{k_m})\prob(\SPB{k+1,m}|b_{k_m},a_{k_m})}{\sum^{M}_{j=1} N(\SPB{k+1,j}) \prob(a_{k_j}|b_{k_j},\pi_{k_j})\prob(\SPB{k+1,m}|b_{k_j},a_{k_j})}$
and plugin them into \ref{eq:q_mcts_mis}
\begin{multline} \label{eq:q_mcts_mis_weights}
	Q_{MIS}(\SB{k},a_k) = \sum^{M}_{m=1}\frac{1}{ N(\SPB{k+1,m})} \cdot \hfill \\ 
	\sum^{ N(\SPB{k+1,m})}_{i=1}\frac{N(\SPB{k+1,m}) \cancel{\prob(a_{k_m}|b_{k_m},\pi_{k_m})}\cancel{\prob(\SPB{k+1,m}|b_{k_m},a_{k_m})}}{\sum^{M}_{j=1} N(\SPB{k+1,j}) \prob(a_{k_j}|b_{k_j},\pi_{k_j})\prob(\SPB{k+1,m}|b_{k_j},\pi_{k_j})} \cdot \hfill \\ \frac{\prob(a_k|b_k,\pi_k)\prob(\SPB{k+1,m}|b_k,a_k)}{\cancel{\prob(a_{k_m}|b_{k_m},\pi_{k_m})}\cancel{\prob(\SPB{k+1,m}|b_{k_m},a_{k_m})}}
	q(\tau_{i,m}(\SB{k},a_k)) = \hfill \\ 
	\sum^{M}_{m=1}\frac{1}{ N(\SPB{k+1,m})} \cdot \hfill \\
	\sum^{ N(\SPB{k+1,m})}_{i=1}\frac{N(\SPB{k+1,m}) \prob(a_k|b_k,\pi_k)\prob(\SPB{k+1,m}|b_k,a_k)}{\sum^{M}_{j=1} N(\SPB{k+1,j}) \prob(a_{k_j}|b_{k_j},\pi_{k_j}) \prob(\SPB{k+1,m}|b_{k_j},a_{k_j})} \cdot \hfill \\ q(\tau_{i,m}(\SB{k},a_k)). \hfill 
\end{multline}

The term $\frac{N(\SPB{k+1,m}) \prob(a_k|b_k,\pi_k)\prob(\SPB{k+1,m}|b_k,a_k)}{\sum^{M}_{j=1} N(\SPB{k+1,j}) \prob(a_{k_j}|b_{k_j},\pi_{k_j}) \prob(\SPB{k+1,m}|b_{k_j},a_{k_j})}$ doesn't depend on i

\begin{multline} \label{eq:q_mcts_mis_weights_final}
	Q_{MIS}(\SB{k},a_k) = \hfill \\ 
	\sum^{M}_{m=1}\frac{1}{ \cancel{N(\SPB{k+1,m})}} \cdot \hfill \\ \frac{ \cancel{N(\SPB{k+1,m})} \prob(a_k|b_k,\pi_k)\prob(\SPB{k+1,m}|b_k,a_k)}{\sum^{M}_{j=1} N(\SPB{k+1,j}) \prob(a_{k_j}|b_{k_j},\pi_{k_j})\prob(\SPB{k+1,m}|b_{k_j},a_{k_j})} \cdot \hfill \\
	\sum^{ N(\SPB{k+1,m})}_{i=1} q(\tau_{i,m}(\SB{k},a_k)) = \hfill \\
	\sum^{M}_{m=1}\frac{ \prob(a_k|b_k,\pi_k)\prob(\SPB{k+1,m}|b_k,a_k)}{\sum^{M}_{j=1} N(\SPB{k+1,j}) \prob(a_{k_j}|b_{k_j},\pi_{k_j}) \prob(\SPB{k+1,m}|b_{k_j},a_{k_j})} \cdot \hfill \\
	\sum^{ N(\SPB{k+1,m})}_{i=1} q(\tau_{i,m}(\SB{k},a_k)) \hfill
\end{multline}

\begin{theorem} \label{recursive_update}
	\textit{The term $\sum^{M}_{m=1}\frac{ \prob(a_k|b_k,\pi_k)\prob(\SPB{k+1,m}|b_k,a_k)}{\sum^{M}_{j=1} N(\SPB{k+1,j}) \prob(a_{k_j}|b_{k_j},\pi_{k_j}) \prob(\SPB{k+1,m}|b_{k_j},a_{k_j})} \cdot \hfill \\
		\sum^{ N(\SPB{k+1,m})}_{i=1} q(\tau_{i,m}(\SB{k},a_k)) \hfill$ can be updated recursively with $O(M)$ complexity given $L$ new samples that originate from same distribution $m'$}.
	\small
\end{theorem}
The derivations above for efficient batch update will be used in out algorithm when we'll choose to reuse certain propagated belief node.

Even though we use Multiple-Importance Sampling estimator to reuse information from previous trajectories, we are aware that they might have originated from different policies and the trajectories came from different distributions. The authors in \cite{Auger13ecml} provide a proof of consistency of the UCT algorithm \cite{Kocsis06ecml} with polynomial exploration for fully observable MDPs with continuous action and state spaces and finite horizon. To our knowledge, there is no proof of consistency of the PFT algorithm \cite{Sunberg18icaps} in the general case of POMDPs with finite horizon and continuous action and state spaces. While the topic presents a promising avenue for future research, the current study focuses on the application and empirical study of using Multiple-Importance Sampling estimator in PFT algorithm.

\subsection{Algorithm}
The algorithm for IR-PFT, is depicted in Algorithms \ref{alg:General} ,\ref{alg:IR-PFT} and \ref{alg:ReuseFunctions} builds upon the principles of PFT \cite{Sunberg18icaps} with notable modifications highlighted in red text. \ref{alg:General} contains a general autonomy loop where the agent plans, executes best action, receives observations from the world and updates reuse candidates for the next planning session. \ref{alg:IR-PFT} is the main part of our algorithm, similarly to PFT, we propagate particle sets through the tree and apply UCT algorithm \cite{Kocsis06ecml} on the belief mdp. In case reuse is possible and current node is root node we first complete needed horizon layers (line 9 in algorithm \ref{alg:IR-PFT}) to fill the horizon gap and then update $Q(b^-_{reuse}), Q(b,a), N(b)$ and $N(ba)$ ($N(b^-_{reuse})$ remains unchanged). The update of $Q(b,a)$ (lines 11 and 31 in algorithm \ref{alg:IR-PFT}) is made using Theorem \ref{recursive_update}. Another change is made in the sampling procedure from existing children nodes according to likelihood in case $|C(ba)|\leq k_o N(ba)^{\alpha_o}$ (line 23 in algorithm \ref{alg:IR-PFT}), since we reuse previous propagated beliefs that came from a different distribution along with propagated beliefs that were generated from the correct distribution we need to correct the likelihood using importance sampling for the reused nodes and then we sample using multinomial distribution . Our solution to determine if we want reused node or open new node was to intermittently take reused node and then open new node (line 2 in ReusePossible method in algorithm \ref{alg:ReuseFunctions}).

Reuse in our algorithm is currently made only for the root node since the potential to save computations is greater - the depth of the root is the smallest in the tree. Reusing for nodes in other depth levels can be done, but isn't in the scope of current work. 

\begin{algorithm}[tb]
	\caption{General Planning Loop}
	\label{alg:General}
	\begin{algorithmic}[1] % [1] shows line numbers
		\STATE \textbf{Procedure}: \textsc{Solve}(b)
		\STATE $\TR \leftarrow \{\}$
		\WHILE{ProblemNotSolved()}
			\STATE $a,\TR' \leftarrow Plan(b,\TR)$ 
			\STATE $o \leftarrow ReceiveObservation(b,a)$
			\STATE $b',b'^-,r \leftarrow G_{PF(m)}(b,a,o)$
			\STATE UpdateReuseCandidates($a, \TR', b, b')$
			\STATE $b \leftarrow b' $
			\STATE $T \leftarrow \TR'$
		\ENDWHILE
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
	\caption{IR-PFT}
	\label{alg:IR-PFT}
	\begin{algorithmic}[1] % [1] shows line numbers
		\STATE \textbf{Procedure}: \textsc{Plan}(b, \TR')
		\FOR {$i \in 1:n$}
		\STATE $Simulate(b, d_{max}, \TR')$
		\ENDFOR
		\STATE $a$ = $argmax_a\{Q(b,a)\}$
		\STATE return $a,\TR$
		\item[]
	\end{algorithmic}
	
	\begin{algorithmic}[1]
		\STATE \textbf{Procedure}: \textsc{Simulate}(b, d, \TR)
		\IF {$d = 0$}
		\STATE return 0
		\ENDIF
		\STATE $a \leftarrow \underset{a \in C(b)}{argmax} \ Q(ba)+c \sqrt{\frac{logN(b)}{N(ba)}} $
		\IF{$|C(ba)|\leq k_oN(ba)^{\alpha_o}$}
		\IF{\textcolor{red}{b is root and ReusePossible(b,a,\TR)}}
		\STATE \textcolor{red}{$\br \leftarrow$ GetReuseCandidate(b,a,\TR)}
		\STATE \textcolor{red}{$Q(\br) \leftarrow$ FillHorizonPropagated(\TR,$\br,d-d_{b^-}$)} 
		\STATE \textcolor{red}{$w(\br) \leftarrow \frac{\prob(\br|b,a)}{\prob(\br|Parent(\br),a)}$}
		\STATE \textcolor{red}{$Q(ba)\leftarrow MISUpdate()$} \COMMENT{update using Theorem \ref{recursive_update}}
		\STATE \textcolor{red}{$N(b) \leftarrow N(b) + N(\br)$}
		\STATE \textcolor{red}{$N(ba) \leftarrow N(ba) + N(\br)$}
		\STATE \textcolor{red}{$C(b,a) \leftarrow C(b,a) \cup \{(\br, w(\br))\}$ }
		\STATE \textcolor{red}{return $total$}
		\ELSE
		\STATE \textcolor{red}{$b',b'^-,r \leftarrow G_{PF(m)}(b,a)$}
		\STATE \textcolor{red}{$C(b,a) \leftarrow C(b,a) \cup \{(b'^-, 1)\}$ }
		\STATE \textcolor{red}{$C(b'^-) \leftarrow C(b'^-) \cup \{(b',r)\}$}
		\STATE $total \leftarrow r + \gamma ROLLOUT(b',d-1)$
		\ENDIF
		\ELSE
		\STATE \textcolor{red}{$b'^- \leftarrow$ sample from $C(ba)$} 
		\STATE \textcolor{red}{$b',r \leftarrow$ sample uniformly from $C(b'^-)$} 
		\STATE $total \leftarrow r + \gamma Simulate(b',d-1,T)$
		\ENDIF
		\STATE $N(b) \leftarrow N(b)+1$
		\STATE \textcolor{red}{$N(b'^-) \leftarrow N(b'^-)+1$}
		\STATE $N(ba) \leftarrow N(ba)+1$
		\STATE $Q(b'^-)\leftarrow Q(ba) + \frac{total-Q(b'^-)}{N(b'^-)}$
		\STATE \textcolor{red}{$Q(ba)\leftarrow MISUpdate()$} \COMMENT{update using Theorem \ref{recursive_update}}
		\STATE return $total$
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
	\caption{Reuse Functions}
	\label{alg:ReuseFunctionsOld}
	\begin{algorithmic}[1] % [1] shows line numbers
		\STATE \textbf{Procedure}: \textsc{UpdateReuseCandidates}(a,\TR,$b_k$,$b^{real}_{k+1}$)
		\STATE ReuseDict $dict \leftarrow$ $\{\}$
		\FOR{$b^-_{k+1} \in C(b_{k},a)$}
			\FOR{$b_{k+1}\in C(b^-_{k+1})$}
				\FOR{$a' \in Actions(b_{k+1})$}
					\FOR{$b^-_{k+2} \in C(b_{k+1},a')$}
						\STATE $dict[a'].append(b^-_{k+2})$
					\ENDFOR	
				\ENDFOR	
			\ENDFOR	
		\ENDFOR
		\STATE $T.SetReuseCandidatesDict(dict)$
		\item[]
	\end{algorithmic}
	\begin{algorithmic}[1]
		\STATE \textbf{Procedure}: \textsc{ReusePossible}(b,a,\TR)
		\IF{$NumReused(b,a)$ mod 2 = 1}
			\STATE return $false$
		\ENDIF
		\STATE $candidates \leftarrow T.GetReuseCandidatesDict()$
		\STATE return not($candidates[a].empty()$)
		\item[]
	\end{algorithmic}

	\begin{algorithmic}[1]
		\STATE \textbf{Procedure}: \textsc{GetReuseCandidate}(b,a,\TR)
		\STATE $candidates \leftarrow GetReuseCandidates(b,a,\TR)$
		\STATE $b^- \leftarrow candidates[a].pop()$
		\STATE return $b^-$
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
	\caption{Fill Horizon Gap}
	\label{alg:AddHorizonLayers}
	\begin{algorithmic}[1] % [1] shows line numbers
		\STATE \textbf{Procedure}: \textsc{FillHorizonPropagated}(\TR,$b^-,d$)
		\STATE $Q_{new}(b^-) \leftarrow 0$
		\FOR{$b' \in C(b^-)$}
			\STATE $Q_{new}(b^-) \leftarrow Q_{new}(b^-) + FillHorizonPosterior(b')$
		\ENDFOR	
		\STATE return $\frac{Q_{new}(b^-)}{N(b^-)}$
		\item[]
	\end{algorithmic}

	\begin{algorithmic}[1] % [1] shows line numbers
	\STATE \textbf{Procedure}: \textsc{FillHorizonPosterior}($b,d$)
	\IF{$IsLeaf(b)$}
		\STATE $a \leftarrow RandomAction()$
		\STATE $b',b'^-,r \leftarrow G_{PF(m)}(b,a)$
		\STATE $N(b,a) \leftarrow 1$
		\STATE $N(b'^-) \leftarrow 1$
		\STATE $Q(b'^-) \leftarrow r$
		\STATE $Q(b,a) \leftarrow r$
		\STATE return $r$
	\ENDIF
	\STATE $Q(b) \leftarrow 0$
	\FOR{$a \in Actions(b)$}
		\FOR{$b'^- \in C(b,a)$}
			\STATE $Q(b) \leftarrow Q(b) + FillHorizonPropagated(b'^-, d-1)$
		\ENDFOR	
	\ENDFOR	
	\STATE $Q(b) \leftarrow \frac{Q(b)}{N(b)}$
	\STATE return $Q(b)$
	\item[]
\end{algorithmic}
\end{algorithm}
UpdateReuseCandidates procedure calculates the set of propagated beliefs that we'll want to have as reuse candidates in future planning sessions. In our implementation the heuristic we used for calculating the set of reused nodes was to add the nodes that we got from executing the same action sequence, but received different observations. 

Figure \ref{fig:reuse_candidates} shows an example of reusing propagated beliefs from previous planning session. The tree in the red rectangle is from planning at time $k$. After the planning session ended, the agent executed chosen action $a_k$ and received real observation from the world $o_{real}$ which led to current belief $\SB{k+1, real}$. Now, during plannig time $k+1$, we consider reusing propagated belief $\SPB{k+2, 1}$ that was sampled from  $\prob(\cdot | \SB{k+1,1},a_{k+1})$ along with $Q(\SPB{k+2, 1})$ and propagated belief $\SPB{k+2, 2}$  that was sampled from  $\prob(\cdot | \SB{k+1,2},a_{k+1})$ along with $Q(\SPB{k+2, 2})$. Both $Q(\SPB{k+2, 1})$ and $Q(\SPB{k+2, 2})$ where calculated with respect to a shorter horizon and we fill this gap in the algorithm. $\SPB{k+2,3}$ was sampled from the correct distribution $\prob(\cdot | \SB{k+1,real},a_{k+1})$ and we have calculated the term  $Q(\SPB{k+2, 3})$ from scratch. The term $Q(\SB{k+1,real},a)$ combines $Q(\SPB{k+2, 1})$, $Q(\SPB{k+2, 2})$ and $Q(\SPB{k+2, 3})$ using Theorem \ref{recursive_update}.

\vspace{-3pt}
\setlength{\belowcaptionskip}{-1pt}
\begin{figure} [!ht]
	\begin{center}
		\centering
		\includegraphics[width=0.8\columnwidth]{./graphics/reuse_candidates.eps}
		\scriptsize
		\caption{\scriptsize Visualization of reused nodes along with new nodes}
		\normalsize
		\label{fig:reuse_candidates_old}
	\end{center}
\end{figure}
\setlength{\belowcaptionskip}{0pt}
FillHorizonPropagated and FillHorizonPosterior procedures extend the previous tree depth to match the depth of the current planning session. The counters $N(b,a), N(b^-), N(b)$ are not changed and $Q(b,a), Q(b^-)$ are updated with the information from the extended horizon.
GetReuseCandidates procedure pops reuse candidate from the set. 
